Rotational Evolution of Classical T Tauri Stars: Models and Observations

We developed a grid of stellar rotation models for low-mass and solar-type Classical T Tauri stars (CTTS) ($0.3M_{\odot}<M_{\ast}<1.2M_{\odot}$). These models incorporate the star-disk interaction and magnetospheric ejections to investigate the evolution of the stellar rotation rate as a function of the mass of the star $M_{\ast}$, the magnetic field ($B_{\ast}$), and stellar wind ($\dot{M}_{wind}$). We compiled and determined stellar parameters for 208 CTTS, such as projected rotational velocity $v\sin(i)$, mass accretion rate $\dot{M}_{acc}$, stellar mass $M_{\ast}$, ages, and estimated rotational periods using TESS data. We also estimated a representative value of the mass-loss rate for our sample using the $[\text{O}\text{ I}]$ spectral line. Our results confirm that $v\sin(i)$ measurements in CTTS agree with the rotation rates provided by our spin models in the accretion-powered stellar winds (APSW) picture. In addition, we used the Approximate Bayesian Computation (ABC) technique to explore the connection between the model parameters and the observational properties of CTTS. We find that the evolution of $v\sin(i)$ with age might be regulated by variations in (1) the intensity of $B_{\ast}$ and (2) the fraction of the accretion flow ejected in magnetic winds, removing angular momentum from these systems. The youngest stars in our sample ($\sim $1 Myr) show a median branching ratio $\dot{M}_{wind}/\dot{M}_{acc}\sim$ $0.16$ and median $B_{\ast}\sim$ 2000 G, in contrast to $\sim 0.01$ and 1000 G, respectively, for stars with ages $\gtrsim 3$ Myr.

==> Table1_complete.tex <==
\begin{deluxetable*}{ccccccccc}
\tablecaption{Stellar parameters of the CTTS sample\label{tab:parameters}}

\tablewidth{0pt}
\tablehead{ \colhead{2MASS ID} & \colhead{$v\sin(i)$\tablenotemark{a}} & \colhead{$M_{\ast}$} & \colhead{Age} & \colhead{$P_{rot}$\tablenotemark{b}} & \colhead{$P_{rot}$\tablenotemark{c}} & \colhead{$\log{\dot{M}_{acc}}$} & \colhead{$\log{\dot{M}_{wind}}$} & \colhead{Binary\tablenotemark{a}} \\
\colhead{} & \colhead{(km~s$^{-1}$)}  &
\colhead{($M_{\odot}$)} & \colhead{(Myr)} & \colhead{(days)} & \colhead{(days)} &
\colhead{($\log$$M_{\odot}$ yr$^{-1}$)} & \colhead{($\log$$M_{\odot}$ yr$^{-1}$)} & 
}
\decimalcolnumbers
\startdata
  05390878-0231115 & 12.8 $\pm$ 0.6 & 0.3 $\pm$ 0.03 & 2.36 $\pm$ 0.53 & \nodata & \nodata & -9.37 $\pm$ 0.31 & -11.13 $\pm$ 0.83 & 1\\
  05380097-0226079 & 16.2 $\pm$ 0.5 & 0.37 $\pm$ 0.03 & 3.77 $\pm$ 0.85 & \nodata & \nodata & -9.01 $\pm$ 0.3 & -10.43 $\pm$ 0.84 & 1\\
  05344178-0453462 & 10.7 $\pm$ 0.7 & 0.44 $\pm$ 0.04 & 1.73 $\pm$ 0.33 & \nodata & \nodata & -8.95 $\pm$ 0.3 & -10.05 $\pm$ 0.84 & 1\\
  05373094-0223427 & 7.7 $\pm$ 0.6 & 0.36 $\pm$ 0.03 & 6.66 $\pm$ 1.46 & \nodata & \nodata & -8.93 $\pm$ 0.3 & -10.38 $\pm$ 0.84 & 1\\
  05391151-0231065 & 13.7 $\pm$ 0.5 & 0.5 $\pm$ 0.04 & 1.3 $\pm$ 0.21 & \nodata & \nodata & -8.89 $\pm$ 0.3 & -9.76 $\pm$ 0.84 & 1\\
  05332852-0517262 & 8.1 $\pm$ 1.2 & 0.5 $\pm$ 0.04 & 1.56 $\pm$ 0.27 & \nodata & \nodata & -8.7 $\pm$ 0.29 & -10.26 $\pm$ 0.83 & 1\\
  05380826-0235562 & 8.8 $\pm$ 0.5 & 0.4 $\pm$ 0.03 & 1.03 $\pm$ 0.18 & \nodata & \nodata & -8.68 $\pm$ 0.29 & -9.9 $\pm$ 0.84 & 1\\
  05384027-0230185 & 18.3 $\pm$ 1.1 & 0.49 $\pm$ 0.03 & 0.8 $\pm$ 0.11 & 7.69 $\pm$ 0.01 & \nodata & -8.67 $\pm$ 0.29 & -9.37 $\pm$ 0.85 & 1\\
  05402461-0152309 & 14.4 $\pm$ 0.5 & 0.54 $\pm$ 0.04 & 1.9 $\pm$ 0.34 & \nodata & \nodata & -8.66 $\pm$ 0.29 & -10.02 $\pm$ 0.84 & 1\\
  05393938-0217045 & 14.1 $\pm$ 0.5 & 0.6 $\pm$ 0.04 & 0.98 $\pm$ 0.16 & \nodata & 13.52 $\pm$ 0.01 & -8.61 $\pm$ 0.29 & -9.93 $\pm$ 0.83 & 1\\
  05343395-0534512 & 22.3 $\pm$ 0.5 & 0.54 $\pm$ 0.04 & 0.82 $\pm$ 0.12 & \nodata & \nodata & -8.56 $\pm$ 0.29 & -9.03 $\pm$ 0.85 & 1\\
  05395362-0233426 & 0.1 $\pm$ 0.6 & 0.35 $\pm$ 0.03 & 2.68 $\pm$ 0.55 & \nodata & \nodata & -8.56 $\pm$ 0.29 & -10.75 $\pm$ 0.83 & 1\\
  05324196-0539239 & 60.7 $\pm$ 1.7 & 0.75 $\pm$ 0.07 & 0.41 $\pm$ 0.07 & 1.7 $\pm$ 0.01 & 1.69 $\pm$ 0.01 & -8.56 $\pm$ 0.29 & -9.29 $\pm$ 0.84 & -1\\
  05400195-0221325 & 8.8 $\pm$ 0.5 & 0.36 $\pm$ 0.03 & 0.96 $\pm$ 0.15 & \nodata & \nodata & -8.54 $\pm$ 0.28 & -10.71 $\pm$ 0.83 & 1\\
  05391883-0230531 & 47.9 $\pm$ 2.6 & 1.1 $\pm$ 0.18 & 2.45 $\pm$ 1.33 & \nodata & 1.83 $\pm$ 0.01 & -8.53 $\pm$ 0.28 & -9.79 $\pm$ 0.83 & -1\\
  05380674-0230227 & 15.3 $\pm$ 2.1 & 0.52 $\pm$ 0.03 & 0.77 $\pm$ 0.11 & \nodata & \nodata & -8.51 $\pm$ 0.28 & -9.05 $\pm$ 0.85 & 1\\
  05401274-0228199 & 50.9 $\pm$ 1.4 & 0.45 $\pm$ 0.03 & 0.52 $\pm$ 0.05 & 1.53 $\pm$ 0.01 & \nodata & -8.49 $\pm$ 0.28 & -10.86 $\pm$ 0.81 & -1\\
  05354600-0057522 & 10.3 $\pm$ 0.7 & 0.65 $\pm$ 0.05 & 1.75 $\pm$ 0.32 & \nodata & \nodata & -8.49 $\pm$ 0.28 & -10.01 $\pm$ 0.83 & 1\tablenotemark{*}\\
  05341420-0542210 & 5.4 $\pm$ 1.1 & 0.62 $\pm$ 0.05 & 2.53 $\pm$ 0.52 & \nodata & \nodata & -8.42 $\pm$ 0.28 & -9.12 $\pm$ 0.85 & 1\\
  05394017-0220480 & 16.1 $\pm$ 0.8 & 0.77 $\pm$ 0.05 & 1.6 $\pm$ 0.27 & 5.8 $\pm$ 0.01 & 5.64 $\pm$ 0.01 & -8.4 $\pm$ 0.28 & -9.73 $\pm$ 0.84 & 1\\
  05292326-0125153 & 22.2 $\pm$ 0.5 & 0.55 $\pm$ 0.05 & 3.15 $\pm$ 0.65 & 2.86 $\pm$ 0.01 & 1.42 $\pm$ 0.01 & -8.35 $\pm$ 0.28 & -9.78 $\pm$ 0.84 & 1\tablenotemark{*}\\
  05322578-0036533 & 10.5 $\pm$ 0.8 & 0.44 $\pm$ 0.03 & 1.09 $\pm$ 0.17 & \nodata & \nodata & -8.34 $\pm$ 0.28 & -9.7 $\pm$ 0.84 & 1\tablenotemark{*}\\
  05345404-0623507 & 7.8 $\pm$ 0.5 & 0.44 $\pm$ 0.03 & 1.02 $\pm$ 0.22 & \nodata & \nodata & -8.3 $\pm$ 0.28 & -9.7 $\pm$ 0.84 & 1\\
  05312062-0049197 & 8.7 $\pm$ 1.5 & 0.18 $\pm$ 0.02 & 1.05 $\pm$ 0.3 & \nodata & 4.96 $\pm$ 0.01 & -8.29 $\pm$ 0.28 & -9.89 $\pm$ 0.85 & 1\tablenotemark{*}\\
  05334545-0536323 & 8.9 $\pm$ 0.6 & 0.29 $\pm$ 0.03 & 0.32 $\pm$ 0.16 & \nodata & \nodata & -8.27 $\pm$ 0.28 & -9.07 $\pm$ 0.86 & 1\\
  05382915-0216156 & 10.8 $\pm$ 0.5 & 0.68 $\pm$ 0.05 & 1.62 $\pm$ 0.31 & \nodata & \nodata & -8.21 $\pm$ 0.27 & -9.86 $\pm$ 0.84 & 1\\
  05393982-0231217 & 4.4 $\pm$ 13.4 & 0.96 $\pm$ 0.12 & 6.3 $\pm$ 3.23 & \nodata & \nodata & -8.19 $\pm$ 0.27 & -8.75 $\pm$ 0.86 & 0\\
  05392935-0227209 & 18.6 $\pm$ 2.2 & 0.31 $\pm$ 0.06 & 2.01 $\pm$ 0.83 & \nodata & \nodata & -8.12 $\pm$ 0.27 & -9.4 $\pm$ 0.86 & 1\\
  05354669-0549262 & 9.7 $\pm$ 0.5 & 0.52 $\pm$ 0.04 & 1.01 $\pm$ 0.15 & \nodata & \nodata & -8.11 $\pm$ 0.27 & -9.7 $\pm$ 0.84 & 1\\
  05390136-0218274 & 7.3 $\pm$ 0.9 & 0.51 $\pm$ 0.04 & 0.91 $\pm$ 0.13 & \nodata & \nodata & -8.09 $\pm$ 0.27 & -9.6 $\pm$ 0.84 & 1\\
  05332136-0521347 & 17.2 $\pm$ 0.9 & 0.66 $\pm$ 0.04 & 0.5 $\pm$ 0.07 & 7.2 $\pm$ 0.01 & 3.7 $\pm$ 2.81 & -7.99 $\pm$ 0.27 & -9.15 $\pm$ 0.84 & 1\\
  05353089-0455178 & 12.6 $\pm$ 0.6 & 0.54 $\pm$ 0.04 & 1.64 $\pm$ 0.3 & \nodata & \nodata & -7.97 $\pm$ 0.27 & -9.74 $\pm$ 0.84 & 1\\
  05340300-0536572 & 30.4 $\pm$ 0.7 & 0.69 $\pm$ 0.05 & 0.29 $\pm$ 0.04 & 2.62 $\pm$ 0.01 & 2.66 $\pm$ 0.01 & -7.78 $\pm$ 0.26 & -8.7 $\pm$ 0.85 & 1\\
  05392519-0238220 & 11.0 $\pm$ 0.5 & 0.55 $\pm$ 0.04 & 0.64 $\pm$ 0.09 & \nodata & \nodata & -7.76 $\pm$ 0.26 & -9.84 $\pm$ 0.83 & 1\\
  05350370-0450530 & 13.4 $\pm$ 1.0 & 0.47 $\pm$ 0.03 & 0.51 $\pm$ 0.05 & \nodata & \nodata & -7.76 $\pm$ 0.26 & -9.5 $\pm$ 0.84 & 1\\
  05344518-0510476 & 9.5 $\pm$ 0.8 & 0.37 $\pm$ 0.03 & 1.03 $\pm$ 0.16 & \nodata & \nodata & -7.73 $\pm$ 0.26 & -9.31 $\pm$ 0.85 & 1\\
  05352262-0514112 & 27.9 $\pm$ 1.5 & 0.43 $\pm$ 0.03 & 0.45 $\pm$ 0.05 & \nodata & \nodata & -7.5 $\pm$ 0.25 & -9.1 $\pm$ 0.85 & 1\\
  05401513-0057266 & 9.5 $\pm$ 0.5 & 0.44 $\pm$ 0.04 & 4.05 $\pm$ 0.95 & \nodata & \nodata & \nodata & \nodata & 1\tablenotemark{*}\\
  05364039-0613334 & 9.9 $\pm$ 0.6 & 0.57 $\pm$ 0.05 & 2.65 $\pm$ 0.56 & \nodata & \nodata & \nodata & \nodata & 1\\
  05353300-0443588 & 17.0 $\pm$ 0.9 & 1.07 $\pm$ 0.05 & 2.67 $\pm$ 0.41 & \nodata & \nodata & \nodata & \nodata & 1\\
  05345833-0554288 & 9.2 $\pm$ 1.1 & 0.46 $\pm$ 0.03 & 1.33 $\pm$ 0.23 & \nodata & \nodata & \nodata & \nodata & 1\\
  05343064-0435526 & 10.6 $\pm$ 0.9 & 0.44 $\pm$ 0.03 & 1.74 $\pm$ 0.32 & \nodata & \nodata & \nodata & \nodata & 1\\
  05333855-0513125 & 8.0 $\pm$ 0.8 & 0.31 $\pm$ 0.03 & 2.17 $\pm$ 0.45 & \nodata & \nodata & \nodata & \nodata & 1\\
  05345559-0555293 & 7.2 $\pm$ 0.6 & 0.34 $\pm$ 0.03 & 1.58 $\pm$ 0.32 & \nodata & \nodata & \nodata & \nodata & 1\\
  05384423-0240197 & 11.4 $\pm$ 1.0 & 0.68 $\pm$ 0.05 & 1.34 $\pm$ 0.24 & \nodata & \nodata & \nodata & \nodata & 1\\
  05350249-0533099 & 31.2 $\pm$ 0.6 & 0.29 $\pm$ 0.03 & 0.93 $\pm$ 0.15 & \nodata & \nodata & \nodata & \nodata & -1\\
  05344441-0526061 & 34.9 $\pm$ 1.1 & 0.15 $\pm$ 0.02 & 0.27 $\pm$ 0.18 & \nodata & \nodata & \nodata & \nodata & -1\\
  05344789-0530465 & 0.1 $\pm$ 1.2 & 0.44 $\pm$ 0.04 & 1.31 $\pm$ 0.23 & \nodata & \nodata & \nodata & \nodata & 1\\
  05372168-0040399 & 1.0 $\pm$ 0.9 & 0.33 $\pm$ 0.03 & 3.08 $\pm$ 0.73 & \nodata & \nodata & \nodata & \nodata & 1\tablenotemark{*}\\
  05215741+0011423 & 4.3 $\pm$ 1.4 & 0.42 $\pm$ 0.04 & 5.08 $\pm$ 1.19 & \nodata & 3.43 $\pm$ 0.01 & \nodata & \nodata & 1\tablenotemark{*}\\
  05400668+0103099 & 4.7 $\pm$ 1.1 & 0.41 $\pm$ 0.04 & 3.58 $\pm$ 0.8 & \nodata & \nodata & \nodata & \nodata & 1\tablenotemark{*}\\
  05352288-0437406 & 4.9 $\pm$ 2.1 & 0.46 $\pm$ 0.04 & 3.24 $\pm$ 0.7 & \nodata & \nodata & \nodata & \nodata & 1\\
  05341320-0533535 & 5.4 $\pm$ 1.1 & 0.49 $\pm$ 0.04 & 5.18 $\pm$ 1.11 & \nodata & \nodata & \nodata & \nodata & 1\\
  05351929-0516447 & 5.8 $\pm$ 4.3 & 0.17 $\pm$ 0.02 & 0.96 $\pm$ 0.39 & 3.75 $\pm$ 0.01 & 3.75 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05353644-0534111 & 6.0 $\pm$ 0.5 & 0.5 $\pm$ 0.04 & 1.16 $\pm$ 0.2 & \nodata & \nodata & \nodata & \nodata & 1\\
  05353733-0623263 & 6.1 $\pm$ 1.1 & 0.42 $\pm$ 0.04 & 2.36 $\pm$ 0.5 & \nodata & \nodata & \nodata & \nodata & 1\\
  05352448-0601463 & 6.3 $\pm$ 1.5 & 0.33 $\pm$ 0.03 & 5.07 $\pm$ 1.07 & 2.95 $\pm$ 0.01 & \nodata & \nodata & \nodata & 1\\
  05344956-0529033 & 6.6 $\pm$ 1.1 & 0.37 $\pm$ 0.03 & 0.63 $\pm$ 0.09 & \nodata & \nodata & \nodata & \nodata & 1\\
  05344514-0621072 & 6.6 $\pm$ 0.5 & 0.4 $\pm$ 0.03 & 2.73 $\pm$ 0.56 & \nodata & \nodata & \nodata & \nodata & 1\\
  05343822-0524236 & 7.0 $\pm$ 1.1 & 0.29 $\pm$ 0.03 & 1.5 $\pm$ 0.31 & \nodata & \nodata & \nodata & \nodata & 1\\
  05344117-0546116 & 7.1 $\pm$ 0.6 & 0.36 $\pm$ 0.03 & 1.21 $\pm$ 0.21 & \nodata & \nodata & \nodata & \nodata & 1\\
  05353079-0530362 & 7.1 $\pm$ 0.9 & 0.26 $\pm$ 0.03 & 0.77 $\pm$ 0.19 & \nodata & \nodata & \nodata & \nodata & 1\\
  05352831-0559132 & 7.2 $\pm$ 0.5 & 0.26 $\pm$ 0.03 & 0.94 $\pm$ 0.18 & \nodata & \nodata & \nodata & \nodata & 1\\
  05344048-0457396 & 7.4 $\pm$ 1.2 & 0.3 $\pm$ 0.03 & 1.89 $\pm$ 0.39 & 2.92 $\pm$ 1.36 & 2.89 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05381315-0245509 & 7.4 $\pm$ 0.6 & 0.45 $\pm$ 0.04 & 1.37 $\pm$ 0.23 & \nodata & \nodata & \nodata & \nodata & 1\\
  05353170-0441077 & 7.7 $\pm$ 2.1 & 0.25 $\pm$ 0.03 & 2.13 $\pm$ 0.54 & \nodata & \nodata & \nodata & \nodata & 1\\
  05353333-0451113 & 7.7 $\pm$ 0.7 & 0.4 $\pm$ 0.04 & 2.23 $\pm$ 0.45 & \nodata & \nodata & \nodata & \nodata & 1\\
  05334167-0524042 & 7.7 $\pm$ 0.8 & 0.41 $\pm$ 0.04 & 3.0 $\pm$ 0.63 & 6.53 $\pm$ 0.06 & 6.81 $\pm$ 0.02 & \nodata & \nodata & 1\\
  05354764-0519145 & 7.7 $\pm$ 1.0 & 0.44 $\pm$ 0.04 & 1.67 $\pm$ 0.35 & \nodata & \nodata & \nodata & \nodata & 1\\
  05352551-0451205 & 7.9 $\pm$ 1.7 & 0.31 $\pm$ 0.03 & 0.98 $\pm$ 0.18 & \nodata & \nodata & \nodata & \nodata & 1\\
  05455311-0013248 & 8.1 $\pm$ 0.5 & 0.46 $\pm$ 0.04 & 2.92 $\pm$ 0.62 & \nodata & \nodata & \nodata & \nodata & 1\\
  05354355-0505414 & 8.3 $\pm$ 0.9 & 0.42 $\pm$ 0.03 & 1.49 $\pm$ 0.28 & \nodata & \nodata & \nodata & \nodata & 1\\
  05454612-0044407 & 8.5 $\pm$ 0.6 & 0.35 $\pm$ 0.03 & 1.65 $\pm$ 0.3 & \nodata & \nodata & \nodata & \nodata & 1\\
  05353070-0518071 & 8.6 $\pm$ 1.1 & 0.32 $\pm$ 0.03 & 0.76 $\pm$ 0.14 & \nodata & \nodata & \nodata & \nodata & 1\\
  05361475-0613169 & 8.7 $\pm$ 0.5 & 0.41 $\pm$ 0.04 & 2.69 $\pm$ 0.59 & \nodata & \nodata & \nodata & \nodata & 1\\
  05291271-0010187 & 8.9 $\pm$ 0.6 & 0.65 $\pm$ 0.05 & 7.04 $\pm$ 1.67 & \nodata & \nodata & \nodata & \nodata & 1\tablenotemark{*}\\
  05385922-0233514 & 9.0 $\pm$ 0.9 & 0.4 $\pm$ 0.03 & 2.14 $\pm$ 0.42 & 4.05 $\pm$ 0.01 & 4.07 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05354049-0452260 & 9.1 $\pm$ 1.0 & 0.36 $\pm$ 0.03 & 2.64 $\pm$ 0.59 & \nodata & \nodata & \nodata & \nodata & 1\\
  05345201-0524187 & 9.3 $\pm$ 0.7 & 0.34 $\pm$ 0.03 & 1.39 $\pm$ 0.26 & 2.35 $\pm$ 0.01 & 2.04 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05345292-0528591 & 9.4 $\pm$ 1.3 & 0.25 $\pm$ 0.03 & 2.24 $\pm$ 0.53 & \nodata & \nodata & \nodata & \nodata & 1\\
  05353672-0510004 & 9.4 $\pm$ 1.5 & 0.21 $\pm$ 0.03 & 1.76 $\pm$ 0.39 & \nodata & \nodata & \nodata & \nodata & 1\\
  05360110-0615314 & 9.5 $\pm$ 1.0 & 0.45 $\pm$ 0.04 & 1.65 $\pm$ 0.3 & \nodata & \nodata & \nodata & \nodata & 1\\
  05333304-0511555 & 9.5 $\pm$ 1.2 & 0.34 $\pm$ 0.03 & 1.58 $\pm$ 0.28 & \nodata & \nodata & \nodata & \nodata & 1\\
  05392030-0118253 & 9.6 $\pm$ 0.6 & 0.29 $\pm$ 0.03 & 1.15 $\pm$ 0.19 & 7.28 $\pm$ 0.02 & \nodata & \nodata & \nodata & 1\tablenotemark{*}\\
  05342587-0456274 & 9.7 $\pm$ 0.6 & 0.42 $\pm$ 0.03 & 1.65 $\pm$ 0.33 & \nodata & \nodata & \nodata & \nodata & 1\\
  05353369-0446237 & 9.7 $\pm$ 0.4 & 0.5 $\pm$ 0.04 & 1.43 $\pm$ 0.26 & \nodata & \nodata & \nodata & \nodata & 1\\
  05351455-0615127 & 9.8 $\pm$ 0.5 & 0.4 $\pm$ 0.03 & 0.77 $\pm$ 0.11 & \nodata & \nodata & \nodata & \nodata & 1\\
  05343005-0449506 & 9.8 $\pm$ 0.9 & 0.55 $\pm$ 0.04 & 1.91 $\pm$ 0.36 & \nodata & \nodata & \nodata & \nodata & 1\\
  05395465-0246341 & 9.8 $\pm$ 0.8 & 0.53 $\pm$ 0.03 & 0.49 $\pm$ 0.06 & \nodata & \nodata & \nodata & \nodata & 1\\
  05385200-0246436 & 9.8 $\pm$ 0.6 & 0.54 $\pm$ 0.04 & 0.95 $\pm$ 0.15 & \nodata & \nodata & \nodata & \nodata & 1\\
  05352804-0517202 & 9.9 $\pm$ 1.1 & 0.19 $\pm$ 0.02 & 0.49 $\pm$ 0.26 & \nodata & \nodata & \nodata & \nodata & 1\\
  05365186-0508358 & 9.9 $\pm$ 0.9 & 0.52 $\pm$ 0.05 & 2.5 $\pm$ 0.53 & 7.78 $\pm$ 0.04 & 7.69 $\pm$ 0.02 & \nodata & \nodata & 1\\
  05342298-0441392 & 9.9 $\pm$ 0.9 & 0.47 $\pm$ 0.03 & 0.91 $\pm$ 0.13 & \nodata & \nodata & \nodata & \nodata & 1\\
  05353178-0023065 & 10.1 $\pm$ 0.6 & 0.41 $\pm$ 0.03 & 1.27 $\pm$ 0.21 & 6.66 $\pm$ 0.02 & 6.92 $\pm$ 0.01 & \nodata & \nodata & 1\tablenotemark{*}\\
  05354413-0448048 & 10.1 $\pm$ 0.9 & 0.5 $\pm$ 0.03 & 1.26 $\pm$ 0.19 & \nodata & 9.7 $\pm$ 0.03 & \nodata & \nodata & 1\\
  05353635-0531378 & 10.1 $\pm$ 0.7 & 0.2 $\pm$ 0.02 & 0.76 $\pm$ 0.28 & \nodata & \nodata & \nodata & \nodata & 1\\
  05352277-0428510 & 10.1 $\pm$ 0.9 & 0.47 $\pm$ 0.04 & 1.86 $\pm$ 0.33 & \nodata & \nodata & \nodata & \nodata & 1\\
  05345073-0527010 & 10.1 $\pm$ 0.7 & 0.58 $\pm$ 0.04 & 1.06 $\pm$ 0.19 & \nodata & \nodata & \nodata & \nodata & 1\\
  05351539-0433262 & 10.3 $\pm$ 0.5 & 0.57 $\pm$ 0.05 & 1.68 $\pm$ 0.3 & \nodata & \nodata & \nodata & \nodata & 1\\
  05392639-0215034 & 10.3 $\pm$ 0.5 & 0.68 $\pm$ 0.05 & 2.4 $\pm$ 0.46 & 6.37 $\pm$ 0.01 & 6.73 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05355462-0527075 & 10.4 $\pm$ 0.4 & 0.47 $\pm$ 0.04 & 1.98 $\pm$ 0.38 & \nodata & \nodata & \nodata & \nodata & 1\\
  05345304-0503271 & 10.5 $\pm$ 1.0 & 0.53 $\pm$ 0.04 & 1.92 $\pm$ 0.35 & \nodata & \nodata & \nodata & \nodata & 1\\
  05354987-0518308 & 10.5 $\pm$ 0.5 & 0.34 $\pm$ 0.03 & 1.2 $\pm$ 0.25 & \nodata & \nodata & \nodata & \nodata & 1\\
  05320040-0140110 & 10.5 $\pm$ 0.5 & 0.68 $\pm$ 0.05 & 4.48 $\pm$ 0.91 & \nodata & \nodata & \nodata & \nodata & 1\tablenotemark{*}\\
  05345156-0525129 & 10.5 $\pm$ 0.8 & 0.54 $\pm$ 0.04 & 0.55 $\pm$ 0.07 & \nodata & \nodata & \nodata & \nodata & 1\\
  05353066-0527167 & 10.5 $\pm$ 1.1 & 0.34 $\pm$ 0.03 & 0.99 $\pm$ 0.17 & \nodata & \nodata & \nodata & \nodata & 1\\
  05353447-0440207 & 10.7 $\pm$ 0.5 & 0.65 $\pm$ 0.05 & 1.43 $\pm$ 0.31 & \nodata & \nodata & \nodata & \nodata & 1\\
  05360808-0441205 & 11.1 $\pm$ 0.9 & 0.45 $\pm$ 0.04 & 1.53 $\pm$ 0.27 & \nodata & \nodata & \nodata & \nodata & 1\\
  05340383-0436062 & 11.2 $\pm$ 0.9 & 0.43 $\pm$ 0.04 & 3.01 $\pm$ 0.63 & \nodata & \nodata & \nodata & \nodata & 1\\
  05343614-0605346 & 11.4 $\pm$ 1.1 & 0.37 $\pm$ 0.03 & 1.92 $\pm$ 0.38 & \nodata & 3.0 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05343266-0521074 & 11.5 $\pm$ 0.4 & 0.46 $\pm$ 0.04 & 2.79 $\pm$ 0.58 & \nodata & \nodata & \nodata & \nodata & 1\\
  05390357-0246269 & 11.5 $\pm$ 0.5 & 0.33 $\pm$ 0.03 & 2.07 $\pm$ 0.49 & 5.05 $\pm$ 0.01 & 5.22 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05352279-0531372 & 11.5 $\pm$ 0.7 & 0.35 $\pm$ 0.03 & 0.76 $\pm$ 0.11 & \nodata & \nodata & \nodata & \nodata & 1\\
  05343024-0511481 & 11.5 $\pm$ 0.7 & 0.46 $\pm$ 0.03 & 0.4 $\pm$ 0.05 & \nodata & \nodata & \nodata & \nodata & 1\\
  05355405-0447193 & 11.5 $\pm$ 1.1 & 0.35 $\pm$ 0.03 & 1.59 $\pm$ 0.28 & \nodata & \nodata & \nodata & \nodata & 1\\
  05321016-0037124 & 11.5 $\pm$ 0.5 & 0.96 $\pm$ 0.05 & 3.72 $\pm$ 0.62 & \nodata & \nodata & \nodata & \nodata & 1\tablenotemark{*}\\
  05345802-0517376 & 11.5 $\pm$ 0.5 & 0.46 $\pm$ 0.04 & 1.41 $\pm$ 0.27 & \nodata & \nodata & \nodata & \nodata & 1\\
  05470696+0000477 & 11.6 $\pm$ 0.3 & 0.58 $\pm$ 0.04 & 0.71 $\pm$ 0.11 & 9.92 $\pm$ 0.02 & \nodata & \nodata & \nodata & 1\\
  05352253-0452369 & 11.6 $\pm$ 0.4 & 0.32 $\pm$ 0.03 & 0.58 $\pm$ 0.16 & 2.78 $\pm$ 0.01 & 2.81 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05334822-0513262 & 11.8 $\pm$ 1.2 & 0.36 $\pm$ 0.03 & 3.19 $\pm$ 0.72 & 4.0 $\pm$ 0.01 & 4.0 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05354886-0612078 & 12.1 $\pm$ 0.4 & 0.73 $\pm$ 0.05 & 0.87 $\pm$ 0.14 & \nodata & \nodata & \nodata & \nodata & 1\\
  05352864-0447265 & 12.1 $\pm$ 0.8 & 0.31 $\pm$ 0.03 & 0.98 $\pm$ 0.16 & \nodata & 4.09 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05354486-0507170 & 12.2 $\pm$ 0.3 & 0.57 $\pm$ 0.03 & 0.17 $\pm$ 0.04 & \nodata & \nodata & \nodata & \nodata & 1\\
  05350167-0432529 & 12.3 $\pm$ 1.0 & 0.44 $\pm$ 0.04 & 3.59 $\pm$ 0.78 & \nodata & \nodata & \nodata & \nodata & 1\\
  05352746-0517099 & 12.5 $\pm$ 0.8 & 0.44 $\pm$ 0.02 & 0.17 $\pm$ 0.05 & \nodata & \nodata & \nodata & \nodata & 1\\
  05352909-0529103 & 12.5 $\pm$ 0.5 & 0.47 $\pm$ 0.03 & 0.59 $\pm$ 0.08 & \nodata & \nodata & \nodata & \nodata & 1\\
  05362788-0625360 & 12.7 $\pm$ 1.1 & 0.19 $\pm$ 0.02 & 1.51 $\pm$ 0.29 & \nodata & \nodata & \nodata & \nodata & 1\\
  05344188-0453382 & 12.7 $\pm$ 1.0 & 0.29 $\pm$ 0.03 & 0.82 $\pm$ 0.15 & \nodata & \nodata & \nodata & \nodata & 1\\
  05351403-0552090 & 12.9 $\pm$ 0.4 & 0.86 $\pm$ 0.05 & 3.83 $\pm$ 0.69 & \nodata & \nodata & \nodata & \nodata & 1\\
  05383902-0245321 & 13.0 $\pm$ 0.5 & 0.4 $\pm$ 0.04 & 2.86 $\pm$ 0.65 & \nodata & \nodata & \nodata & \nodata & 1\\
  05474836+0040589 & 13.1 $\pm$ 0.3 & 0.45 $\pm$ 0.03 & 0.5 $\pm$ 0.06 & 7.36 $\pm$ 0.01 & 7.56 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05352459-0511296 & 13.2 $\pm$ 0.7 & 0.46 $\pm$ 0.03 & 0.65 $\pm$ 0.09 & \nodata & \nodata & \nodata & \nodata & 1\\
  05353528-0521271 & 13.3 $\pm$ 1.0 & 0.55 $\pm$ 0.08 & 17.53 $\pm$ 27.86 & \nodata & \nodata & \nodata & \nodata & 1\\
  05455738+0020222 & 13.5 $\pm$ 0.4 & 0.54 $\pm$ 0.04 & 0.69 $\pm$ 0.1 & \nodata & \nodata & \nodata & \nodata & 1\\
  05342572-0456554 & 13.6 $\pm$ 0.8 & 0.75 $\pm$ 0.05 & 1.89 $\pm$ 0.39 & \nodata & \nodata & \nodata & \nodata & 1\\
  05352157-0509497 & 13.6 $\pm$ 0.8 & 0.34 $\pm$ 0.03 & 3.62 $\pm$ 0.83 & \nodata & \nodata & \nodata & \nodata & 1\\
  05373003-0048520 & 13.7 $\pm$ 0.9 & 0.6 $\pm$ 0.05 & 1.56 $\pm$ 0.29 & \nodata & \nodata & \nodata & \nodata & 1\tablenotemark{*}\\
  05360729-0542216 & 13.7 $\pm$ 1.0 & 0.74 $\pm$ 0.05 & 1.37 $\pm$ 0.23 & 2.06 $\pm$ 0.01 & 2.05 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05355225-0443048 & 13.9 $\pm$ 0.4 & 0.62 $\pm$ 0.05 & 2.07 $\pm$ 0.4 & \nodata & \nodata & \nodata & \nodata & 1\\
  05400889-0233336 & 14.3 $\pm$ 0.7 & 0.54 $\pm$ 0.04 & 0.66 $\pm$ 0.1 & 5.99 $\pm$ 0.01 & \nodata & \nodata & \nodata & 1\\
  05360665-0614259 & 14.3 $\pm$ 0.3 & 0.56 $\pm$ 0.04 & 1.21 $\pm$ 0.21 & 8.31 $\pm$ 0.01 & \nodata & \nodata & \nodata & 1\\
  05392927+0003390 & 14.8 $\pm$ 0.5 & 0.78 $\pm$ 0.05 & 2.38 $\pm$ 0.43 & 3.68 $\pm$ 0.01 & \nodata & \nodata & \nodata & 1\tablenotemark{*}\\
  05351632-0515380 & 14.9 $\pm$ 0.8 & 0.59 $\pm$ 0.04 & 0.74 $\pm$ 0.13 & \nodata & \nodata & \nodata & \nodata & 1\\
  05352169-0534468 & 15.1 $\pm$ 0.9 & 0.48 $\pm$ 0.03 & 0.65 $\pm$ 0.08 & \nodata & \nodata & \nodata & \nodata & 1\\
  05355765-0557183 & 15.3 $\pm$ 0.9 & 0.47 $\pm$ 0.04 & 1.87 $\pm$ 0.33 & \nodata & \nodata & \nodata & \nodata & 1\\
  05345651-0527510 & 15.4 $\pm$ 0.4 & 0.43 $\pm$ 0.04 & 2.07 $\pm$ 0.41 & \nodata & \nodata & \nodata & \nodata & 1\\
  05361584-0614507 & 15.5 $\pm$ 0.6 & 0.41 $\pm$ 0.04 & 4.41 $\pm$ 0.98 & 3.48 $\pm$ 0.01 & \nodata & \nodata & \nodata & 1\\
  05342978-0451477 & 15.9 $\pm$ 0.9 & 0.71 $\pm$ 0.05 & 8.32 $\pm$ 1.79 & \nodata & \nodata & \nodata & \nodata & 1\\
  05352372-0448166 & 15.9 $\pm$ 0.7 & 0.21 $\pm$ 0.03 & 1.78 $\pm$ 0.37 & \nodata & \nodata & \nodata & \nodata & 1\\
  05361847-0620387 & 16.0 $\pm$ 0.4 & 0.51 $\pm$ 0.04 & 2.6 $\pm$ 0.52 & \nodata & \nodata & \nodata & \nodata & 1\\
  05351784-0444524 & 16.0 $\pm$ 1.0 & 0.63 $\pm$ 0.05 & 1.43 $\pm$ 0.26 & 1.56 $\pm$ 0.01 & 1.56 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05350822-0537047 & 16.0 $\pm$ 0.8 & 0.44 $\pm$ 0.03 & 0.61 $\pm$ 0.08 & 3.79 $\pm$ 0.01 & 7.65 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05353560-0515432 & 16.1 $\pm$ 0.5 & 0.4 $\pm$ 0.03 & 0.76 $\pm$ 0.1 & \nodata & \nodata & \nodata & \nodata & 1\\
  05350460-0458289 & 16.3 $\pm$ 0.9 & 0.76 $\pm$ 0.03 & 12.72 $\pm$ 3.22 & \nodata & \nodata & \nodata & \nodata & 1\\
  05341262-0450247 & 16.9 $\pm$ 0.4 & 0.82 $\pm$ 0.05 & 0.58 $\pm$ 0.08 & 5.61 $\pm$ 0.01 & 5.49 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05333982-0038541 & 17.4 $\pm$ 0.9 & 0.75 $\pm$ 0.05 & 3.94 $\pm$ 0.84 & \nodata & \nodata & \nodata & \nodata & 1\tablenotemark{*}\\
  05343371-0540227 & 17.5 $\pm$ 0.6 & 0.24 $\pm$ 0.03 & 0.89 $\pm$ 0.21 & \nodata & \nodata & \nodata & \nodata & 1\\
  05351885-0444100 & 17.6 $\pm$ 0.9 & 0.15 $\pm$ 0.02 & 0.51 $\pm$ 0.35 & 1.56 $\pm$ 0.01 & \nodata & \nodata & \nodata & 1\\
  05350585-0448432 & 17.7 $\pm$ 0.7 & 0.65 $\pm$ 0.05 & 2.56 $\pm$ 0.5 & \nodata & \nodata & \nodata & \nodata & 1\\
  05350801-0532442 & 17.8 $\pm$ 0.5 & 0.63 $\pm$ 0.05 & 1.71 $\pm$ 0.35 & 6.73 $\pm$ 0.02 & 6.51 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05303164+0203051 & 17.9 $\pm$ 0.4 & 0.62 $\pm$ 0.05 & 2.46 $\pm$ 0.47 & 4.52 $\pm$ 0.01 & 4.7 $\pm$ 0.01 & \nodata & \nodata & 1\tablenotemark{*}\\
  05350052-0601235 & 18.0 $\pm$ 1.4 & 0.41 $\pm$ 0.04 & 4.71 $\pm$ 1.05 & \nodata & \nodata & \nodata & \nodata & 1\\
  05352791-0614150 & 18.3 $\pm$ 1.1 & 0.66 $\pm$ 0.05 & 2.45 $\pm$ 0.5 & \nodata & \nodata & \nodata & \nodata & 1\\
  05354764-0537388 & 18.6 $\pm$ 0.6 & 0.23 $\pm$ 0.03 & 1.11 $\pm$ 0.24 & \nodata & \nodata & \nodata & \nodata & 1\\
  05333148-0609541 & 18.6 $\pm$ 0.6 & 0.27 $\pm$ 0.03 & 0.92 $\pm$ 0.17 & 3.51 $\pm$ 0.01 & \nodata & \nodata & \nodata & 1\\
  05354986-0446323 & 18.8 $\pm$ 1.1 & 0.3 $\pm$ 0.03 & 1.09 $\pm$ 0.2 & \nodata & \nodata & \nodata & \nodata & 1\\
  05382725-0245096 & 18.9 $\pm$ 0.7 & 0.5 $\pm$ 0.04 & 1.33 $\pm$ 0.24 & \nodata & \nodata & \nodata & \nodata & 1\\
  05274199-0144217 & 18.9 $\pm$ 0.6 & 0.82 $\pm$ 0.05 & 2.72 $\pm$ 0.47 & 4.52 $\pm$ 0.01 & 4.6 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05390297-0241272 & 19.0 $\pm$ 0.5 & 0.41 $\pm$ 0.03 & 1.36 $\pm$ 0.24 & \nodata & \nodata & \nodata & \nodata & 1\\
  05322569-0157112 & 19.1 $\pm$ 0.4 & 0.74 $\pm$ 0.05 & 5.57 $\pm$ 1.25 & 3.89 $\pm$ 0.01 & 3.7 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05341138-0451229 & 19.1 $\pm$ 0.9 & 0.42 $\pm$ 0.03 & 1.89 $\pm$ 0.34 & \nodata & \nodata & \nodata & \nodata & 1\\
  05355077-0516291 & 19.2 $\pm$ 0.7 & 0.75 $\pm$ 0.05 & 1.37 $\pm$ 0.23 & \nodata & \nodata & \nodata & \nodata & 1\\
  05342949-0513551 & 19.6 $\pm$ 0.7 & 0.7 $\pm$ 0.06 & 2.41 $\pm$ 0.57 & \nodata & \nodata & \nodata & \nodata & 1\\
  05382750-0235041 & 19.8 $\pm$ 0.6 & 0.35 $\pm$ 0.03 & 2.24 $\pm$ 0.46 & \nodata & \nodata & \nodata & \nodata & 1\\
  05350900-0427510 & 20.0 $\pm$ 1.0 & 1.29 $\pm$ 0.09 & 2.07 $\pm$ 0.4 & 7.16 $\pm$ 0.01 & 7.91 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05244103+0154386 & 20.1 $\pm$ 0.5 & 0.6 $\pm$ 0.05 & 7.08 $\pm$ 1.74 & 4.78 $\pm$ 0.01 & 4.78 $\pm$ 0.01 & \nodata & \nodata & 1\tablenotemark{*}\\
  05362611-0608038 & 20.3 $\pm$ 0.4 & 0.48 $\pm$ 0.03 & 0.46 $\pm$ 0.05 & \nodata & \nodata & \nodata & \nodata & 1\\
  05352673-0516451 & 21.1 $\pm$ 1.8 & 0.29 $\pm$ 0.03 & 2.27 $\pm$ 0.57 & \nodata & \nodata & \nodata & \nodata & 1\\
  05360508-0629321 & 21.5 $\pm$ 0.4 & 0.82 $\pm$ 0.03 & 10.93 $\pm$ 2.15 & 7.61 $\pm$ 0.01 & 7.69 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05344753-0557569 & 22.0 $\pm$ 0.5 & 0.64 $\pm$ 0.04 & 0.64 $\pm$ 0.09 & \nodata & \nodata & \nodata & \nodata & 1\\
  05345044-0520203 & 22.3 $\pm$ 1.0 & 0.51 $\pm$ 0.04 & 1.08 $\pm$ 0.19 & 3.34 $\pm$ 0.01 & 3.29 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05351852-0513383 & 22.7 $\pm$ 0.6 & 0.46 $\pm$ 0.02 & 0.14 $\pm$ 0.03 & \nodata & \nodata & \nodata & \nodata & 1\\
  05353217-0511579 & 23.2 $\pm$ 1.1 & 0.28 $\pm$ 0.03 & 0.89 $\pm$ 0.17 & \nodata & \nodata & \nodata & \nodata & 1\\
  05342792-0526346 & 23.5 $\pm$ 0.6 & 0.66 $\pm$ 0.05 & 3.37 $\pm$ 0.76 & \nodata & \nodata & \nodata & \nodata & 1\\
  05355018-0521169 & 23.5 $\pm$ 1.2 & 0.29 $\pm$ 0.04 & 2.45 $\pm$ 0.65 & \nodata & \nodata & \nodata & \nodata & 1\\
  05363616-0555288 & 24.2 $\pm$ 0.5 & 0.55 $\pm$ 0.04 & 0.78 $\pm$ 0.11 & \nodata & \nodata & \nodata & \nodata & 1\\
  05355433-0526444 & 24.4 $\pm$ 0.6 & 0.53 $\pm$ 0.04 & 1.78 $\pm$ 0.32 & 4.4 $\pm$ 0.01 & 4.03 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05371885-0020416 & 24.4 $\pm$ 0.9 & 1.08 $\pm$ 0.05 & 3.47 $\pm$ 0.57 & 2.47 $\pm$ 0.01 & 2.43 $\pm$ 0.01 & \nodata & \nodata & 1\tablenotemark{*}\\
  05215426-0217257 & 25.5 $\pm$ 1.0 & 0.91 $\pm$ 0.05 & 2.35 $\pm$ 0.47 & \nodata & \nodata & \nodata & \nodata & 1\\
  05344907-0526266 & 27.8 $\pm$ 1.5 & 0.31 $\pm$ 0.05 & 2.92 $\pm$ 0.95 & \nodata & \nodata & \nodata & \nodata & 1\\
  05413275-0157574 & 27.8 $\pm$ 0.5 & 0.5 $\pm$ 0.04 & 2.63 $\pm$ 0.51 & \nodata & \nodata & \nodata & \nodata & 1\tablenotemark{*}\\
  05350873-0504407 & 29.4 $\pm$ 1.0 & 0.23 $\pm$ 0.02 & 0.43 $\pm$ 0.22 & \nodata & \nodata & \nodata & \nodata & 1\\
  05415220-0201211 & 29.8 $\pm$ 0.9 & 0.84 $\pm$ 0.05 & 0.26 $\pm$ 0.03 & 2.26 $\pm$ 0.01 & \nodata & \nodata & \nodata & 1\tablenotemark{*}\\
  05350576-0533558 & 31.1 $\pm$ 0.7 & 0.31 $\pm$ 0.03 & 0.54 $\pm$ 0.16 & \nodata & \nodata & \nodata & \nodata & 1\\
  05462243-0008526 & 31.1 $\pm$ 0.4 & 1.06 $\pm$ 0.06 & 1.8 $\pm$ 0.29 & \nodata & \nodata & \nodata & \nodata & 1\\
  05351809-0515461 & 35.1 $\pm$ 1.4 & 0.36 $\pm$ 0.05 & 2.7 $\pm$ 0.85 & \nodata & \nodata & \nodata & \nodata & 1\\
  05351790-0542340 & 40.5 $\pm$ 0.7 & 0.66 $\pm$ 0.05 & 0.28 $\pm$ 0.03 & 5.31 $\pm$ 0.01 & 5.77 $\pm$ 0.01 & \nodata & \nodata & 1\\
  05345737-0514334 & 41.2 $\pm$ 1.0 & 0.37 $\pm$ 0.03 & 1.98 $\pm$ 0.44 & \nodata & \nodata & \nodata & \nodata & 1\\
  05341954-0530198 & 43.3 $\pm$ 1.1 & 1.14 $\pm$ 0.12 & 1.26 $\pm$ 0.33 & \nodata & \nodata & \nodata & \nodata & 1\\
  05352016-0526390 & 56.5 $\pm$ 1.6 & 0.67 $\pm$ 0.05 & 0.29 $\pm$ 0.03 & \nodata & \nodata & \nodata & \nodata & 1\\
  05365983-0120245 & 21.3 $\pm$ 1.7 & 0.27 $\pm$ 0.03 & 1.37 $\pm$ 0.31 & \nodata & \nodata & \nodata & \nodata & 2\tablenotemark{*}\\
  05350392-0529033 & 30.7 $\pm$ 0.7 & 0.48 $\pm$ 0.03 & 0.52 $\pm$ 0.06 & \nodata & \nodata & \nodata & \nodata & 2\\
  05320638-0111000 & 40.0 $\pm$ 0.9 & 0.35 $\pm$ 0.03 & 0.97 $\pm$ 0.15 & \nodata & \nodata & \nodata & \nodata & 2\tablenotemark{*}\\
  05351121-0517209 & 55.3 $\pm$ 1.9 & 0.45 $\pm$ 0.03 & 0.68 $\pm$ 0.09 & \nodata & \nodata & \nodata & \nodata & 2\\
  05354311-0424556 & 56.8 $\pm$ 1.5 & 0.56 $\pm$ 0.04 & 0.7 $\pm$ 0.11 & \nodata & \nodata & \nodata & \nodata & 2\\
  05414141-0143533 & 66.6 $\pm$ 2.0 & 2.2 $\pm$ 0.09 & 0.83 $\pm$ 0.12 & \nodata & \nodata & \nodata & \nodata & 2\\
  05351236-0543184 & 99.9 $\pm$ 1.8 & 0.65 $\pm$ 0.05 & 1.0 $\pm$ 0.17 & \nodata & \nodata & \nodata & \nodata & 2\\
  05395428-0224385 & 83.9 $\pm$ 3.4 & 0.39 $\pm$ 0.03 & 0.34 $\pm$ 0.1 & \nodata & \nodata & \nodata & \nodata & 3\\
\enddata
\tablenotetext{a}{\citet{Kounkel_2018,Kounkel_2019}: 0- Undeconvolvable cross-correlation function (CCF); 1- Only a single component in the CCF; 2- Multiple components in the CCF; -1- Spotted pairs or SB2 Uncertain}
\tablenotetext{b}{TESS Sector 6}
\tablenotetext{c}{TESS Sector 32}
\tablenotetext{*}{\citet{Tokovinin_2020} visual binaries}
\tablecomments{Only a portion of the table is shown here. The full version is available in electronic form.}
\end{deluxetable*}
